Nested smoothing algorithms for inference and tracking of heterogeneous multi-scale state-space systems

Multi-scale problems, where variables of interest evolve in different time-scales and live in different state-spaces, can be found in many fields of science. Here, we introduce a new recursive methodology for Bayesian inference that aims at estimating the static parameters and tracking the dynamic variables of these kind of systems. Although the proposed approach works in rather general multi-scale systems, for clarity we analyze the case of a heterogeneous multi-scale model with 3 time-scales (static parameters, slow dynamic state variables and fast dynamic state variables). The proposed scheme, based on nested filtering methodology of P\'erez-Vieites et al. (2018), combines three intertwined layers of filtering techniques that approximate recursively the joint posterior probability distribution of the parameters and both sets of dynamic state variables given a sequence of partial and noisy observations. We explore the use of sequential Monte Carlo schemes in the first and second layers while we use an unscented Kalman filter to obtain a Gaussian approximation of the posterior probability distribution of the fast variables in the third layer. Some numerical results are presented for a stochastic two-scale Lorenz 96 model with unknown parameters.

==> src/myfile1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
xmin=0.1,
xmax=0.9,
xlabel={rho},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
ymin=-8,
ymax=4,
ylabel={C(nats)},
axis background/.style={fill=white},
title={Upper and Lower Bound Special Case},
legend style={legend cell align=left,align=left,draw=black}
]
\addplot [color=blue,solid]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addlegendentry{UB};

\addplot [color=red,solid]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\addlegendentry{LB};

\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.1	2.30258509299405\\
0.2	1.6094379124341\\
0.3	1.20397280432594\\
0.4	0.916290731874155\\
0.5	0.693147180559945\\
0.6	0.510825623765991\\
0.7	0.356674943938732\\
0.8	0.22314355131421\\
0.9	0.105360515657826\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.1	-0.768753876800411\\
0.2	-2.22587429048891\\
0.3	-3.15418045910748\\
0.4	-3.87551862340106\\
0.5	-4.49918900118285\\
0.6	-5.08366987795047\\
0.7	-5.67728532410536\\
0.8	-6.34803354089389\\
0.9	-7.27536040685204\\
};
\end{axis}
\end{tikzpicture}%
